Metric-Fair Classifier Derandomization

We study the problem of classifier derandomization in machine learning: given a stochastic binary classifier $f: X \to [0,1]$, sample a deterministic classifier $\hat{f}: X \to \{0,1\}$ that approximates the output of $f$ in aggregate over any data distribution. Recent work revealed how to efficiently derandomize a stochastic classifier with strong output approximation guarantees, but at the cost of individual fairness -- that is, if $f$ treated similar inputs similarly, $\hat{f}$ did not. In this paper, we initiate a systematic study of classifier derandomization with metric fairness guarantees. We show that the prior derandomization approach is almost maximally metric-unfair, and that a simple ``random threshold'' derandomization achieves optimal fairness preservation but with weaker output approximation. We then devise a derandomization procedure that provides an appealing tradeoff between these two: if $f$ is $\alpha$-metric fair according to a metric $d$ with a locality-sensitive hash (LSH) family, then our derandomized $\hat{f}$ is, with high probability, $O(\alpha)$-metric fair and a close approximation of $f$. We also prove generic results applicable to all (fair and unfair) classifier derandomization procedures, including a bias-variance decomposition and reductions between various notions of metric fairness.

==> omitted_sections/binary_features.tex <==
%========================================================================================
\section{Binary Features}
%========================================================================================
In this section we consider the special case in which the features are all binary, i.e. the classifier is a Boolean function $f: \{0,1\}^n \to \{0,1\}$.


%========================================================================================
\subsection{Harper's Theorem}
Harper's theorem gives the solution to the isoperimetry problem on the hypercube; in particular, it shows that the subgraph of the $d$-dimensional hypercube with maximum vertex boundary per unit volume is the Hamming ball. An implication of the original theorem, due to Leader (1991), says that
\begin{theorem}
For any set $S$ such that $|S| \geq \sum _{i=0}^r \binom{d}{i}$, we have $|S \cup \partial(S)| \geq \sum_{i=0}^{r+1}\binom{d}{i}$.
\end{theorem}

This theorem can be used to infer that for the hypercube on $n$ vertices, the boundary of any non-trivial set must be $\Theta(n)$. \\

Question: In the hypercube setting, does it make sense to think of, as an analogue for Lipschitz classifiers, classifiers that have bounded difference in output for points that are neighbors? This would then naturally extend to longer distances as well. Under this setting, using a similar cost function, it could make sense to look at what is a profitable manipulation, and then use the size of the boundary to make a statement about the result in expectation. \\

We want to design a distribution of Boolean functions $\calF$ such that
\begin{align*}
    \forall x \in X,
    \quad
    \Pr_{\hat{f} \in \calF}\left[x \text{ can game } \hat{f}\right] \quad \text{is small}
\end{align*}

The following shows an inherent limit to this goal:

\begin{theorem}[Lower bound on gamability for binary feature vectors]
\label{theorem:lower-bound-on-binary-points-on-boundary}
Given a weakly balanced deterministic classifier $f: \{0,1\}^n \to \{0,1\}$ (i.e. there exists a constant $\delta \in (0,1)$ such that $\Pr[f(x)=1] = \delta$), there exist $\Omega\left(\frac{2^n}{\sqrt{n}}\right)$ points (i.e. an $\Omega(1/\sqrt{n})$ fraction) that are on to the decision boundary, i.e. such points can flip their decision by changing just one coordinate.
\end{theorem}
\begin{proof}[Proof sketch]
Harper's theorem plus linearity of expectation.
\end{proof}

\begin{remark}
A \emph{dictator function} is a Boolean function whose output depends only on one feature, i.e. $f(x) = x_i$ for some $i \in [n]$. In this case, every vertex is on the decision boundary.
\end{remark}


%========================================================================================
\subsection{Notions of Manipulation}
Here are two notions of manipulation for the binary feature setting:
\begin{enumerate}
    \item The fraction of players who can game the system by changing $1$ (or $k$) feature(s). (Theorem \ref{theorem:lower-bound-on-binary-points-on-boundary} is a result along these lines.)
    \item The number of ways a player can game the system. This corresponds to \emph{edge} isoperimetry.
\end{enumerate}

Question: Can we show the impossibility of simultaneously preventing both kinds of manipulation?

==> omitted_sections/experiments.tex <==
%========================================================================================
\section{Experiments}
%========================================================================================
\jimmy{What kind of experiments should we do? Ideally, should include some comparison of loss/accuracy measures as well as individual fairness parameters between the following:
\begin{enumerate}
    \item A stochastic classifier $f$ for some task
    \item Our derandomization of $f$, denoted $\hat{f}_{\mathrm{LSH}}$
    \item The CNG pairwise-independent derandomization $\hat{f}_{\mathrm{PI}}$
\end{enumerate}
Comparing loss functions is straightforward (also, look at CNG paper to see how they evaluated loss approximation). But a tricky question is how to measure the fairness parameters $\alpha$ and $\beta$. One idea is to measure ``empirical'' fairness parameters as follows: given a (stochastic or deterministic) classifier $f$ and dataset $x_1,\ldots,x_N$, suppose we fix an empirical $\beta$, denoted $\hat{\beta} \in [0,1]$. Then the corresponding empirical $\alpha$ is
\begin{align*}
    \hat{\alpha} := \frac{1}{\binom{N}{2}} \sum_{x \neq x' \in X} \hat{\alpha}_{x,x'}
    \qquad \text{where} \qquad
    \hat{\alpha}_{x,x'} := \max\left(\frac{|f(x) - f(x')| - \hat{\beta}}{d(x,x')}, 0\right)
\end{align*}
On the other hand, if we fix $\hat{\alpha} \geq 0$, then
\begin{align*}
    \hat{\beta} := \frac{1}{\binom{N}{2}} \sum_{x \neq x' \in X} \hat{\beta}_{x,x'}
    \qquad \text{where} \qquad
    \hat{\beta}_{x,x'} := \max(|f(x) - f(x')| - \hat{\alpha} \cdot d(x,x'), 0)
\end{align*}
This gives fairness \emph{curves} for $f$, $\hat{f}_{\mathrm{LSH}}$, and $\hat{f}_{\mathrm{PI}}$ over data $\{x_i\}$; for each classifier, we can:
\begin{itemize}
    \item Display this curve visually ($\hat{\alpha}$ on the x-axis, $\hat{\beta}$ on the y-axis)
    \item Calculate the AUC, with the hope that $AUC(f) \lesssim AUC(\hat{f}_{\mathrm{LSH}}) \ll AUC(\hat{f}_{\mathrm{PI}})$
\end{itemize}
}

==> omitted_sections/summaries_of_related_work.tex <==
%========================================================================================
\section{Summaries of Related Work}
%========================================================================================

%========================================================================================
\subsection{CGN: Derandomization via Pairwise Independence}
Here we sketch the prior classifier derandomization approach of Cotter, Narasimhan, and Gupta \cite{cotter2019making}. The core construction and analysis happens in Lemma 1 in the appendix:

\begin{lemma}[Output approximation of pairwise-independent derandomization (simplified Lemma 1 of \cite{cotter2019making})]
Let $f$ be a stochastic classifier, $\ell$ a loss function, $\calD$ a distribution over $X$, and $\calH_\PI$ a pairwise-independent hash family. For each $h_\PI \in \calH_\PI$, define the deterministic classifier
\begin{align} \label{equation:f-hat}
    \hat{f}_{h_\PI}(x) = \Indicator \left\{ f(x) \geq \frac{h_\PI(x)}{k} \right\}
\end{align}

Recall the definition of error $E_\ell(f)$ in the main part of the paper. Then
\begin{align}
    \mathrm{bias}(\ell,f,\hat{f})
    &:= \left| E_\ell(f) - \E_{h_\PI \sim \calH_\PI} \left[E_\ell(\hat{f}_{h_\PI})\right] \right|
    \leq \frac{1}{k} \\
    \mathrm{variance}(\ell,\hat{f})
    &:= \Var_{h_\PI \sim \calH_\PI} \left[E_\ell(\hat{f}_{h_\PI})\right]
    \leq \sum_{x \in X} \Pr_{x \sim \calD}[x]^2 \cdot \left[f(x)(1-f(x)) + \frac{1}{k}\right]
\end{align}
\end{lemma}

Intuitively, this construction uses a pairwise independent hash function $h_\PI$ to generate a pseudo-random number $h_\PI(x) \in [k]$, so that $\hat{f}_{h_\PI}$ is a threshold function where each $x \in X$ gets its own threshold $\frac{h_\PI(x)}{k} \in [0,1]$. Here, assume that $X$ is a finite set. This allows us to ignore their awkward clustering scheme $\pi: X \to \calC$, which changes nothing fundamental.

\begin{proof}
Define the \emph{bucketed} stochastic classifier
\begin{align*}
    g(x) = \frac{1}{k} \sum_{i=1}^k \Indicator \left\{ f(x) \geq \frac{i}{k} \right\}
\end{align*}
In other words, $g(x)$ is the smallest multiple of $1/k$ greater than $f(x)$. $g$ is therefore a conceptual half-step between $f$ and $\E_h[\hat{f}_h]$ in that it is essentially discretized, but still fine-grained enough that $|g(x)-f(x)| \leq \frac{1}{k}$ for all $x$. \\

Now define the \emph{deterministic} classifier $\hat{g}_h$ from $g$ just as $\hat{f}$ was defined from $f$ in \eqref{equation:f-hat}, i.e.
\begin{align*}
    \hat{g}_h(x) = \Indicator \left\{ g(x) \geq \frac{h(x)}{k} \right\}
\end{align*}

It essentially suffices to analyze $\hat{g}_h$ instead of $\hat{f}_h$, since in the end, we simply incur an additional bias of $\frac{1}{k}$. The analysis of $\hat{f}_h$ is split into two parts: \\

\textbf{Bias:} Observe that $\Pr_{h \sim \mathcal{H}} \left[\hat{g}_h(x)=1\right] = g(x)$, i.e. $\mathrm{bias}(\ell,g,\hat{g}) = 0$ for any loss function $\ell$. This immediately implies that $\mathrm{bias}(\ell,f,\hat{f}) \leq \frac{1}{k}$. Note that this depends only on $\mathcal{H}$ being uniform, and not on it being pairwise independent. \\

\textbf{Variance:} Recall the notation that the loss of a stochastic classifier $f$ on a data point $(x,y)$ is
\begin{align*}
    L(f,x,y) := f(x)\ell(1,y) + (1-f(x))\ell(0,y)
\end{align*}

Note that
\begin{align*}
    \mathrm{variance}(\ell,\hat{f})
    = \mathrm{variance}(\ell,\hat{g})
    := \Var_{h \sim \calH} \left[E_\ell(\hat{g}_h)\right]
    = \E_{h \sim \calH} \left[E_{\hat{g}_h}(\ell)^2\right] - E_{g}(\ell)^2
\end{align*}

We consider the first term:
\begin{align*}
    & \E_{h \sim \calH} \left[ E_{\hat{g}_h}(\ell)^2 \right] \\
    &= \E_{h \sim \calH} \left[
            \E_{(x,y) \sim \calD} [\ell(\hat{g}_h(x),y)]^2
        \right] \\
    &= \E_{h \sim \calH} \left[
            \E_{(x,y), (x',y') \sim \calD} [
                \ell(\hat{g}_h(x),y) \ell(\hat{g}_h(x'),y')
            ]
        \right] \\
    &= \E_{h \sim \calH} \left[
            \E_{\substack{(x,y), \\ (x',y')}} [
                \Indicator\{\pi(x) = \pi(x')\}
                \ell(\hat{g}_h(x),y) \ell(\hat{g}_h(x'),y')
            ]
        \right]
        + \E_{h \sim \calH} \left[
            \E_{\substack{(x,y), \\ (x',y')}} [
                \Indicator\{\pi(x) \neq \pi(x')\}
                \ell(\hat{g}_h(x),y) \ell(\hat{g}_h(x'),y')
            ]
        \right] \\
    &= \E_{h \sim \calH} \left[
            \E_{\substack{(x,y), \\ (x',y')}} [
                \Indicator\{\pi(x) = \pi(x')\}
                \ell(\hat{g}_h(x),y) \ell(\hat{g}_h(x'),y')
            ]
        \right]
        + \E_{\substack{(x,y), \\ (x',y')}} [
            \Indicator\{\pi(x) \neq \pi(x')\}
            L(g,x,y) L(g,x',y')
        ]
\end{align*}
where the last step follows from the pairwise independence of $\calH$. Next consider the second term:
\begin{align*}
    E_g(\ell)^2
    &= \E_{(x,y) \sim \calD} [L(g,x,y)]^2 \\
    &= \E_{(x,y), (x',y') \sim \calD} [
            L(g,x,y)
            L(g,x',y')
        ]
\end{align*}

Putting these together, we have
\begin{align*}
    & \variance(\hat{f},\ell) \\
    &= \E_{h \sim \calH} \left[
            \E_{\substack{(x,y), \\ (x',y')}} [
                \Indicator\{\pi(x) = \pi(x')\}
                \ell(\hat{g}_h(x),y) \ell(\hat{g}_h(x'),y')
            ]
        \right]
        - \E_{\substack{(x,y), \\ (x',y')}} \left[
            \Indicator\{\pi(x) = \pi(x')\}
            L(g,x,y) L(g,x',y')
        \right] \\
    &= \E_{\substack{(x,y), \\ (x',y')}} \left[
            \Indicator\{\pi(x) = \pi(x')\} \cdot \left(
                \E_{h} [
                    \ell(\hat{g}_h(x),y) \ell(\hat{g}_h(x'),y')
                ]
                - L(g,x,y) L(g,x',y')
            \right)
        \right] \\
    &= \E_{\substack{(x,y), \\ (x',y')}} \left[
            \Indicator\{\pi(x) = \pi(x')\} \cdot \left(
                \E_{h} [
                    \ell(\hat{g}_h(x),y) \ell(\hat{g}_h(x'),y')
                ]
                - \E_{h} [\ell(\hat{g}_h(x),y)]
                \E_{h} [\ell(\hat{g}_h(x'),y')]
            \right)
        \right] \\
    &= \E_{\substack{(x,y), \\ (x',y')}} \left[
            \Indicator\{\pi(x) = \pi(x')\} \cdot
            \Cov_{h \sim \calH} \left(
                \ell(\hat{g}_h(x),y), \ell(\hat{g}_h(x'),y')
            \right)
        \right] \\
    &\leq \E_{\substack{(x,y), \\ (x',y')}} \left[
            \Indicator\{\pi(x) = \pi(x')\} \cdot
            \sqrt{
                \Var_{h \sim \calH} \left(\ell(\hat{g}_h(x),y)\right)
                \Var_{h \sim \calH} \left(\ell(\hat{g}_h(x'),y')\right)
            }
        \right]
        \tag{Cauchy-Schwarz inequality} \\
    &= \sum_{c \in \calC} \left(
            \E_{(x,y)} \left[
                \Indicator\{\pi(x) = c\} \cdot
                \sqrt{
                    \Var_{h \sim \calH} \left(\ell(\hat{g}_h(x),y)\right)
                }
            \right]
        \right)^2 \\
    &= \sum_{c \in \calC} \left(
            \Pr_{x \sim \calD} [\pi(x) = c]
            \cdot
            \E_{(x,y)} \left[
                \sqrt{
                    \Var_{h \sim \calH} \left(\ell(\hat{g}_h(x),y)\right)
                }
                ~ \middle| ~
                \pi(x) = c
            \right]
        \right)^2 \\
    &\leq \sum_{c \in \calC}
        \left(
                \Pr_{x \sim \calD} [\pi(x) = c]
            \right)^2
        \cdot \E_{(x,y)} \left[
            \Var_{h \sim \calH} \left(\ell(\hat{g}_h(x),y)\right)
            ~ \middle| ~
            \pi(x) = c
        \right]
        \tag{Jensen's inequality} \\
    &\leq \sum_{c \in \calC}
        \left(
                \Pr_{x \sim \calD} [\pi(x) = c]
            \right)^2
        \cdot \E_x \left[
            \Var_{h \sim \calH} \left(\hat{g}_h(x)\right)
            ~ \middle| ~
            \pi(x) = c
        \right]
        \tag{since $\ell$ is binary, either $\Var_{\fhat}(\ell(\fhat(x),y)) = \Var_{\fhat}(\fhat(x))$ or $\Var_{\fhat}(\ell(\fhat(x),y)) = 0$} \\
    &\leq \sum_{c \in \calC}
        \left(
                \Pr_{x \sim \calD} [\pi(x) = c]
            \right)^2
        \cdot \E_x [
            g(x)(1-g(x))
            ~|~
            \pi(x) = c
        ] \\
    &\leq \sum_{c \in \calC}
        \left(
                \Pr_{x \sim \calD} [\pi(x) = c]
            \right)^2
        \cdot \left(
            \E_x [
                f(x)(1-f(x))
                ~|~
                \pi(x) = c
            ]
            + \frac{1}{k}
        \right)
        \tag{$\mathrm{bias}(\ell,f,g) \leq \frac{1}{k}$}
\end{align*}
If desired, this can be simplified to
\begin{align*}
    \variance(\hat{f},\ell)
    \leq \max_{b \in B} \Pr_{x \sim \calD} [\pi(x) = b]
        \cdot \E_{x \sim \calD} [f(x)(1-f(x))]
        + \frac{1}{k}
\end{align*}
\end{proof}
Observe that this bound is at its maximum (over possible $\pi$ and $\calD$) when there exists some $c \in \calC$ such that $\Pr_{x \sim \calD}[\pi(x)=c] = 1$, in which case
\begin{align*}
    \variance(\ell,\hat{f})
    \approx \E_{x \sim \calD} [f(x)(1-f(x))]
    \approx \E_{x \sim \calD} \left[\Var_{f} (f(x))\right]
\end{align*}
The bound is sharpest when $\Pr_{x \sim \calD}[\pi(x)=c] = 1/|\calC|$ for all $c \in \calC$, in which case
\begin{align*}
    \variance(\ell,\hat{f})
    = O\left(\frac{1}{|\calC|}\right)
\end{align*}



\begin{proof}[Unfinished alternative variance bound]
To evaluate the first term, note that for any $x,x' \in X$ and $y,y' \in \{0,1\}$,
\begin{align*}
    & \E_{\substack{h_\LS \sim \calH_\LS \\ h_\PI \sim \calH_\PI}} \left[
            \ell(\hat{g}(x),y) \ell(\hat{g}(x'),y')
        \right] \\
    =& \E_{\substack{h_\LS \sim \calH_\LS \\ h_\PI \sim \calH_\PI}} [
            \ell(\hat{g}(x),y) \ell(\hat{g}(x'),y')
            ~|~
            h_\LS(x) = h_\LS(x')
        ]
        \cdot \Pr_{h_\LS \sim \calH_\LS} [h_\LS(x) = h_\LS(x')] \\
        &\qquad
        + \E_{\substack{h_\LS \sim \calH_\LS \\ h_\PI \sim \calH_\PI}} [
            \ell(\hat{g}(x),y) \ell(\hat{g}(x'),y')
            ~|~
            h_\LS(x) \neq h_\LS(x')
        ]
        \cdot \Pr_{h_\LS \sim \calH_\LS} [h_\LS(x) \neq h_\LS(x')] \\
    =& \E_{\substack{h_\LS \sim \calH_\LS \\ h_\PI \sim \calH_\PI}} [
            \ell(\hat{g}(x),y) \ell(\hat{g}(x'),y')
            ~|~
            h_\LS(x) = h_\LS(x')
        ]
        \cdot \phi(x,x') \\
        &\qquad
        + \E_{\substack{h_\LS \sim \calH_\LS \\ h_\PI \sim \calH_\PI}} [
            \ell(\hat{g}(x),y) \ell(\hat{g}(x'),y')
            ~|~
            h_\LS(x) \neq h_\LS(x')
        ]
        \cdot d(x,x')
        \tag{locality sensitivity} \\
    =& \E_{\substack{h_\LS \sim \calH_\LS \\ h_\PI \sim \calH_\PI}} [
            \ell(\hat{g}(x),y) \ell(\hat{g}(x'),y')
            ~|~
            h_\LS(x) = h_\LS(x')
        ]
        \cdot \phi(x,x') \\
        &\qquad
        + \E_{\substack{h_\LS \sim \calH_\LS \\ h_\PI \sim \calH_\PI}} [
            \ell(\hat{g}(x),y)
            ~|~
            h_\LS(x) \neq h_\LS(x')
        ]
        \cdot \E_{\substack{h_\LS \sim \calH_\LS \\ h_\PI \sim \calH_\PI}} [
            \ell(\hat{g}(x'),y')
            ~|~
            h_\LS(x) \neq h_\LS(x')
        ]
        \cdot d(x,x')
        \tag{pairwise independence} \\
    =& \E_{\substack{h_\LS \sim \calH_\LS \\ h_\PI \sim \calH_\PI}} [
            \ell(\hat{g}(x),y) \ell(\hat{g}(x'),y')
            ~|~
            h_\LS(x) = h_\LS(x')
        ]
        \cdot \phi(x,x')
        + L(g,x,y) L(g,x',y') \cdot d(x,x')
        \tag{$\calH_\PI$ is uniform}
\end{align*}
Thus the first term of the variance is
\begin{align*}
    & \E_{\substack{h_\LS \sim \calH_\LS \\ h_\PI \sim \calH_\PI}} \left[
            E_\ell(\hat{g})^2
        \right] \\
    =& \E_{\substack{h_\LS \sim \calH_\LS \\ h_\PI \sim \calH_\PI}} \left[
            \left(
                \E_{(x,y) \sim \calD} [\ell(\hat{g}(x),y)]
            \right)^2
        \right] \\
    =& \E_{\substack{h_\LS \sim \calH_\LS \\ h_\PI \sim \calH_\PI}} \left[
            \E_{\substack{(x,y) \sim \calD \\ (x',y') \sim \calD}} [
                \ell(\hat{g}(x),y) \ell(\hat{g}(x'),y')
            ]
        \right] \\
    =& \E_{\substack{(x,y) \sim \calD \\ (x',y') \sim \calD}} \left[
            \E_{\substack{h_\LS \sim \calH_\LS \\ h_\PI \sim \calH_\PI}} [
                \ell(\hat{g}(x),y) \ell(\hat{g}(x'),y')
            ]
        \right] \\
    =& \E_{\substack{(x,y) \sim \calD \\ (x',y') \sim \calD}} \left[
            \E_{\substack{h_\LS \sim \calH_\LS \\ h_\PI \sim \calH_\PI}} [
                \ell(\hat{g}(x),y) \ell(\hat{g}(x'),y')
                ~|~
                h_\LS(x) = h_\LS(x')
            ]
            \cdot \phi(x,x')
            + L(g,x,y) L(g,x',y') \cdot d(x,x')
        \right]
\end{align*}
\end{proof}


\newpage
%========================================================================================
\subsection{Braverman-Garg: Manipulation-Proof Classifiers}
Braverman and Garg \cite{braverman2020role} provide a condition for a stochastic classifier $f$ to be manipulation-proof:

\begin{definition}[1-Lipschitz classifier]
A randomized classifier $f$ is \emph{1-Lipschitz with respect to a cost function $c$}, or $f \in \mathrm{Lip}_1(c)$, if for all $x,x' \in X$,
\begin{align}
    f(x') - f(x) \leq c(x, x')
\end{align}
\end{definition}

\begin{proposition}
If $f \in \mathrm{Lip}_1(c)$, then no individual is incentivized to change their features even if they have full knowledge of $f$.
\end{proposition}
\begin{proof}
Suppose $f \in \mathrm{Lip}_1(c)$. Consider an individual with original features $x$ who changes their features to any other $x'$. Observe that by Lipschitzness, their utility does not increase:
\begin{align*}
    U(x, x') = f(x') - c(x,x') \leq f(x) = U(x, x)
\end{align*}
\end{proof}

They then show that there exist good classifiers for the class of \emph{simple} cost functions:

\begin{definition}[simple cost function]
A cost function $c: X \times X \to \mathbb{R}$ is \emph{simple} if:
\begin{enumerate}
    \item Costs are non-negative: $c(x,x') \geq 0$ for all $x,x' \in X$.
    
    \item Reducing your qualification is free: if $y(x) \geq y(x')$, then $c(x,x') = 0$.
    \jw{note that due to this condition, simple cost functions are not metrics.}
    
    \item Triangle inequality: $c(x,x'') \leq c(x,x') + c(x',x'')$ for all $x,x',x'' \in X$.
\end{enumerate}
\end{definition}

\begin{theorem}[informal Theorem 3 of Braverman-Garg]
For every simple cost function $c$, there exists a randomized classifier $f \in \mathrm{Lip}_1(c)$ that maximizes the ``efficiency'' (defined in their paper).
\end{theorem}

\jw{TODO: investigate whether the above 1-Lipschitz stochastic classifier can be combined with our derandomization. I no longer think this works, because simple cost functions are not metrics.}

==> omitted_sections/unused_results.tex <==
%========================================================================================
\section{Unused Results}
%========================================================================================

%========================================================================================
\subsection{Uniform Locality-Sensitive Hashing}
\begin{lemma}[LSH families can be made uniform]
\label{lemma:LSH-families-can-be-made-uniform}
For any family $\calH$ of hash functions $h: X \to [k]$, there exists a hash family $\calH'$ with the following properties:
\begin{enumerate}
    \item $\calH'$ preserves $\calH$'s collision rates (and hence, if $\calH$ is an LSH family, its locality-sensitivity): for all $x, x' \in X$,
    \begin{align*}
        \Pr_{h' \sim \calH'} \left[h'(x) = h'(x')\right]
        = \Pr_{h \sim \calH} \left[h(x) = h(x')\right]
    \end{align*}
    
    \item $\calH'$ has the following uniformity properties: for all $x \neq x' \in X$ and $i \in [k]$,
    \begin{align*}
        \Pr_{h' \sim \calH'} \left[h'(x) = i ~\middle|~ h'(x) = h'(x')\right]
        = \Pr_{h' \sim \calH'} \left[h'(x) = i ~\middle|~ h'(x) > h'(x')\right]
        = \Pr_{h' \sim \calH'} \left[h'(x) = i\right]
        = \frac{1}{k}
    \end{align*}
    
    \item $\calH'$ is symmetric: for all $x, x' \in X$,
    \begin{align*}
        \Pr_{h' \sim \calH'} [h'(x) > h'(x')]
        = \Pr_{h' \sim \calH'} [h'(x) < h'(x')]
    \end{align*}
    
    \item $\calH'$ has size $2k \cdot |\calH|$, and can be sampled with $O(\log k)$ more random bits than $\calH$.
\end{enumerate}
\end{lemma}

\begin{proof}
We define a family $\calH'$ that contains $2k$ hash functions for each one in $\calH$. In particular, for each $h \in \calH$, $\calH'$ contains $h_1',\ldots,h_k'$ and $h_{-1}',\ldots,h_{-k}'$, where
\begin{align*}
    h_1'(x) &:= h(x) + 1 \text{ (mod $k$)} + 1
        & h_{-1}'(x) &:= k + 1 - h_1'(x) \\
    h_2'(x) &:= h(x) + 2 \text{ (mod $k$)} + 1
        & h_{-2}'(x) &:= k + 1 - h_2'(x) \\
            & \ \ \vdots & & \ \ \vdots \\
    h_k'(x) &:= h(x) + k \text{ (mod $k$)} + 1
        & h_{-k}'(x) &:= k + 1 - h_k'(x)
\end{align*}

For the rest of the proof, fix some $x,x' \in X$, let $[\pm k] := \{-k,\ldots,-1,1,\ldots,k\}$, and note that all sampling is done uniformly. To see property 1, consider some $h \in \calH$; since the functions $\left\{h_j' ~\middle|~ j \in [\pm k]\right\}$ are simply permuted versions of $h$, they collide precisely when $h$ does:
\begin{align} \label{equation:permuted-hash-functions-preserve-collisions}
    h(x) = h(x')
    \iff h_j'(x) = h_j'(x')
        \quad \forall j \in [\pm k]
\end{align}

We prove property 2 by first demonstrating a more general fact: that even if $\calH'$ were constructed from some \emph{subset} of $\calH$, it would still be uniform. To that end, fix any $i \in [k]$ and $H \subseteq \calH$. We have
\begin{align*}
    \Pr_{h_j' \sim \calH'} \left[h_j'(x) = i ~\middle|~ h \in H\right]
    = \Pr_{\substack{h \sim H \\ j \sim [\pm k]}} \left[h_j'(x) = i\right]
    = \sum_{h \in H} \Pr_{j \sim [\pm k]} \left[h_j'(x) = i ~\middle|~ h\right]
        \cdot \Pr_{h \sim H}[h]
    = \Pr_{j \sim [\pm k]} \left[h_j'(x) = i ~\middle|~ h\right]
\end{align*}
Now observe that exactly one function among $h_1',\ldots,h_k'$, plus one among $h_{-1}',\ldots,h_{-k}'$, maps $x$ to bucket $i$. Thus
\begin{align*}
    \Pr_{j \sim [\pm k]} \left[h_j'(x) = i ~\middle|~ h\right]
    = \frac{2}{2k}
    = \frac{1}{k}
\end{align*}
Setting $H$ to $\{h \in \calH ~|~ h(x) = h(x')\}$, $\{h \in \calH ~|~ h(x) > h(x')\}$, or $\calH$ and applying \eqref{equation:permuted-hash-functions-preserve-collisions} yields property 2. For property 3, observe for every $h \in \calH$ and $j \in [k]$,
\begin{align*}
    h_j'(x) < h_j'(x')
    \quad \Longleftrightarrow \quad
    h_{-j}'(x) > h_{-j}'(x')
\end{align*}
In other words, there are an equal number of functions in $\calH'$ that make the inequality go either way; hence 
\begin{align*}
    \Pr_{h' \sim \calH'} [h'(x) > h'(x')]
    = \Pr_{h' \sim \calH'} [h'(x) < h'(x')]
    = \frac{1}{2} \Pr_{h' \sim \calH'} [h'(x) \neq h'(x')]
\end{align*}

Lastly for property 4, $\calH'$ can be sampled uniformly by sampling $h \sim \calH$ and, using $O(\log k)$ additional random bits, $j \sim [\pm k]$.
\end{proof}


%========================================================================================
\subsection{Composition with LSH Preserves Lipschitzness in Expectation}
\begin{lemma}[Composing a function with LSH preserves Lipschitzness in expectation]
\label{lemma:LSH-preserves-lipschitzness}
Suppose $f: X \to \mathbb{R}$ is $L$-Lipschitz with respect to distance function $d: X \times X \to [0,1]$, and suppose $\mathcal H$ is an LSH family for $d$ containing functions $h: X \to X$ (that is, $k = |X|$, so that each bucket corresponds to some $x \in X$). Then
\begin{align*}
    \E_h[ |f(h(x)) - f(h(x'))| ] \leq L \cdot d(x,x') \label{composition}
\end{align*}
\end{lemma}

As usual, this bound can be made to hold approximately with high probability, by repeatedly evaluating $f$ on many independently-sampled hash functions.

\begin{proof}
We have
\begin{align}
    \E_h[ |f(h(x)) - f(h(x'))| ]
    &= \E_h[ |f(h(x)) - f(h(x'))| ~|~ h(x) = h(x')] \cdot \Pr_h[h(x) = h(x')] \\
    &\quad + \E_h[ |f(h(x)) - f(h(x'))| ~|~ h(x) \neq h(x')] \cdot \Pr_h[h(x) \neq h(x')]
\end{align}
The first term is zero, since $f(h(x)) - f(h(x')) = 0$ when $h(x) = h(x')$. We therefore have
\begin{align*}
    \E_h[ |f(h(x)) - f(h(x'))| ]
    &= \E_h[ |f(h(x)) - f(h(x'))| ~|~ h(x) \neq h(x')] \cdot \Pr_h[h(x) \neq h(x')] \\
    &= \E_h[ |f(h(x)) - f(h(x'))| ~|~ h(x) \neq h(x')] \cdot d(x,x')
        \tag{$h$ is LSH} \\
    &\leq L \cdot d(h(x),h(x')) \cdot d(x,x')
        \tag{$f$ is Lipschitz} \\
    &\leq L \cdot d(x,x')
        \tag{$d(\cdot,\cdot) \leq 1$}
\end{align*}
\end{proof}

==> work_in_progress/random_threshold_variance.tex <==
%========================================================================================
\section{Variance of the Random Threshold Derandomization}
%========================================================================================
\cref{proposition:random-threshold-derandomization-guarantees} claims bounds on the fairness preservation, bias, and variance of the random threshold derandomization
\begin{align*}
    \calF_\RT := \left\{\hat{f}_r ~\middle|~ r \in [0,1]\right\},
    \quad \text{where} \quad
    \hat{f}_r := \Indicator\{f(x) \geq r\}
\end{align*}

The pointwise and aggregate bias are both zero, since for any $x \in X$,
\begin{align*}
    \E_{\hat{f}_r \sim \calF_\RT} \left[
            \hat{f}_r(x)
        \right]
    = \Pr_{r \sim [0,1]} [f(x) \geq r]
    = f(x)
\end{align*}

However, we previously claimed to have an exact expression for the variance, whose proof contained a mistake:
\begin{claim}[Incorrect]
\label{claim:incorrect-variance}
$
    \variance(\hat{f}_r,\calD)
    = \E_{x \sim \calD}[f(x)(1 - f(x))]
$.
\end{claim}
\begin{proof}[Incorrect proof]
We have
\begin{align*}
    \variance(\hat{f}_r,\calD)
    &:= \Var_{\hat{f}_r \sim \calF_\RT} \left(
            \E_{x \sim \calD} \left[
                \hat{f}_r(x)
            \right]
        \right) \\
    &= \E_{x \sim \calD} \left[
             \Var_{\hat{f}_r \sim \calF_\RT} \left(
                \hat{f}_r(x)
            \right)
        \right]
        \tag{{\color{red}incorrect step}} \\
    &= \E_{x \sim \calD} \left[
            \E_{r \sim [0,1]} \left[
                \hat{f}_r(x)
            \right]
            \left(
                1 - \E_{r \sim [0,1]} \left[
                    \hat{f}_r(x)
                \right]
            \right)
        \right] \\
    &= \E_{x \sim \calD} [f(x)(1 - f(x))].
\end{align*}
\end{proof}

Here is a correct bound, no longer an equality:
\begin{claim}[Correct]
\label{claim:correct-variance}
$
    \variance(\hat{f}_r,\calD)
    \leq \E_{x \sim \calD}[f(x)] (1 - \E_{x \sim \calD}[f(x)])
$.
\end{claim}
\begin{proof}[Correct proof]
\begin{align*}
    \variance(\hat{f}_r,\calD)
    &:= \Var_{\hat{f}_r \sim \calF_\RT} \left(
            \E_{x \sim \calD} \left[
                \hat{f}_r(x)
            \right]
        \right) \\
    &= \E_{r \sim [0,1]} \left[
            \left(
                \E_{x \sim \calD} \left[
                    \hat{f}_r(x)
                \right]
            \right)^2
        \right]
        - \left(
            \E_{r \sim [0,1]} \left[
                \E_{x \sim \calD} \left[
                    \hat{f}_r(x)
                \right]
            \right]
        \right)^2 \\
    &\leq \E_{r \sim [0,1]} \left[
            \E_{x \sim \calD} \left[
                \hat{f}_r(x)
            \right]
        \right]
        - \left(
            \E_{r \sim [0,1]} \left[
                \E_{x \sim \calD} \left[
                    \hat{f}_r(x)
                \right]
            \right]
        \right)^2
        \tag{$0 \leq \E_{x \sim \calD} [\hat{f}_r(x)] \leq 1$} \\
    &= \E_{x \sim \calD} \left[
            \E_{r \sim [0,1]} \left[
                \hat{f}_r(x)
            \right]
        \right]
        - \left(
            \E_{x \sim \calD} \left[
                \E_{r \sim [0,1]} \left[
                    \hat{f}_r(x)
                \right]
            \right]
        \right)^2 \\
    &= \E_{x \sim \calD} [f(x)]
        - \left(
            \E_{x \sim \calD} [f(x)]
        \right)^2 \\
    &= \E_{x \sim \calD}[f(x)]
        \left(
            1 - \E_{x \sim \calD}[f(x)]
        \right)
\end{align*}
\end{proof}


\begin{proof}[another proof by Yang]
\begin{align*}
    \variance(\hat{f}_r,\calD)
    &:= \Var_{\hat{f}_r \sim \calF_\RT} \left(
            \E_{x \sim \calD} \left[
                \hat{f}_r(x)
            \right]
        \right) \\
    &= \E_{r \sim [0,1]} \left[
            \left(
                \E_{x \sim \calD} \left[\hat{f}_r(x)\right]
            \right)^2
        \right]
        - \left(
            \E_{r \sim [0,1]} \left[
                \E_{x \sim \calD} \left[
                    \hat{f}_r(x)
                \right]
            \right]
        \right)^2 \\
    &\leq \E_{r \sim [0,1]} \left[
            \E_{x \sim \calD} \left[
                \left(\hat{f}_r(x)\right)^2
            \right]
        \right]
        - \left(
            \E_{r \sim [0,1]} \left[
                \E_{x \sim \calD} \left[
                    \hat{f}_r(x)
                \right]
            \right]
        \right)^2
        \tag{Jensen's inequality for the first term $\E[f(X)] \geq f(E[X])$ when $f$ is convex} \\
    &=\E_{r,x} \left[
            \left(\hat{f}_r(x)\right)^2
        \right]
        - \left(
            \E_{r,x}\left[ \hat{f}_r(x)\right]
        \right)^2 \\
    &= \E_{r,x}\left[
            \left(
                \hat{f}_r(x)
                - \E_{r,x} \left[\hat{f}_r(x)\right]
            \right)^2
        \right] \\
    &=\E_{r,x} \left[
            \E_{r,x}\left[
                \left(
                    \hat{f}_r(x)
                    - \E_{r,x} \left[\hat{f}_r(x)\right]
                \right)^2
             ~\middle|~
            x \right]
        \right] \tag{tower property by treating $    \left(
                    \hat{f}_r(x)
                    - \E_{r,x} \left[\hat{f}_r(x)\right]
                \right)^2$ as the random variable }\\
    &=\E_{r,x} \left[
            f(x) \cdot (1-f(x))^2
            + (1-f(x)) \cdot (0-f(x))^2
        \right]
        \tag{given $x$, the only randomness is in $r$} \\
    &\text{\yc{The above line is incorrect because $\E_{r,x}[\hat{f}_r(x)]$ is a fixed number rather than a function of $x$}}\\ &\text{\yc{thus $\E_{r,x}[\hat{f}_r(x)] = \E_x[f(x)]\neq f(x)$ even conditioned on $x$}}\\    
    &=\E_{r,x} \left[
            f(x) \cdot (1-f(x)) \cdot (1-f(x)+f(x))
        \right] \\
    &=\E_{r,x} \left[
            f(x) \cdot (1-f(x))
        \right] \\
  %  &=\E_{r,x} \left[
  %          f(x) \cdot (1-f(x))
  %      \right]
   %     \tag{using the tower property again for $\E[\E[f(x)(1-f(x))|x]]$} \\
    &=\E_{x} \left[
            f(x) \cdot (1-f(x))
        \right]
        \tag{no randomness in $r$ anymore, dropping $r$}
\end{align*}
\end{proof}


In terms of presenting our paper, the problem with using the latter bound is not just that it's quantitatively looser. The bigger issue is that since it's only an \emph{upper} bound on the variance of $\calF_\RT$, we can no longer definitively say that $\calF_\PI$ or $\calF_\LS$ have lower variance than $\calF_\RT$.

The correct bound is looser than the incorrectly proven one, with the gap at its largest in the following case:
\begin{example}
Suppose we are given $f$ and $\calD$ such that
\begin{align*}
    \Pr_{x \sim \calD} [f(x) = 1] = \frac{1}{2}
    \qquad \textrm{and} \qquad
    \Pr_{x \sim \calD} [f(x) = 0] = \frac{1}{2}
\end{align*}
Then it can be checked that the correct bound, \cref{claim:correct-variance}, says $\variance(\hat{f}_r,\calD) \leq \frac{1}{4}$, while the \emph{incorrectly} proven \cref{claim:incorrect-variance} says (correctly in this case!) that $\variance(\hat{f}_r,\calD) = 0$.
\end{example}

Here are some possibly true statements, in decreasing order of desirability for our presentation. Note that a counterexample to any of these can be given by specifying a stochastic classifier $f$ and data distribuation $\calD$.
\begin{enumerate}
    \item Perhaps \cref{claim:incorrect-variance} is actually correct; that is,
        \begin{align*}
            \E_{r \sim [0,1]} \left[
                    \left(
                        \E_{x \sim \calD} \left[
                            \hat{f}_r(x)
                        \right]
                    \right)^2
                \right]
                - \left(
                    \E_{x \sim \calD} [f(x)]
                \right)^2
            = \E_{x \sim \calD} [f(x)(1 - f(x))]
        \end{align*}
    \item Perhaps the \emph{lower bound} part of it is correct, i.e.
        \begin{align*}
            \variance(\hat{f}_r,\calD) \geq \E_{x \sim \calD}[f(x)(1 - f(x))]
        \end{align*}
        since this allows us to state that other derandomizations have lower variance in general.
    \item Perhaps the \emph{upper bound} part of it is correct, i.e.
        \begin{align*}
            \variance(\hat{f}_r,\calD) \leq \E_{x \sim \calD}[f(x)(1 - f(x))]
        \end{align*}
        This would still be nice to know, since $\E_{x \sim \calD}[f(x)(1 - f(x))]$ is a worst-case variance for the other two derandomizations as well.
\end{enumerate}

If none of these turn out to be true (or easily provable), one easy way out is to simply use \cref{claim:correct-variance} and point out that there are cases when this bound is tight (namely when $f$ is a constant function over the support of $\calD$).


